MolCA: Molecular Graph-Language Modeling with Cross-Modal Projector and Uni-Modal Adapter

Language Models (LMs) have demonstrated impressive molecule understanding ability on various 1D text-related tasks. However, they inherently lack 2D graph perception - a critical ability of human professionals in comprehending molecules' topological structures. To bridge this gap, we propose MolCA: Molecular Graph-Language Modeling with Cross-Modal Projector and Uni-Modal Adapter. MolCA enables an LM (e.g., Galactica) to understand both text- and graph-based molecular contents via the cross-modal projector. Specifically, the cross-modal projector is implemented as a Q-Former to connect a graph encoder's representation space and an LM's text space. Further, MolCA employs a uni-modal adapter (i.e., LoRA) for the LM's efficient adaptation to downstream tasks. Unlike previous studies that couple an LM with a graph encoder via cross-modal contrastive learning, MolCA retains the LM's ability of open-ended text generation and augments it with 2D graph information. To showcase its effectiveness, we extensively benchmark MolCA on tasks of molecule captioning, IUPAC name prediction, and molecule-text retrieval, on which MolCA significantly outperforms the baselines. Our codes and checkpoints can be found at https://github.com/acharkq/MolCA.

==> chapters/introduction.tex <==
\section{Introduction}
% % context. 
% Para1: LLMs have achieved extensive successes in many areas. In particular, due to the extensive biochemical literature in their pretraining data, LLMs have learned chemistry concepts and obtained the high-level understanding of molecule properties~\citep{GPT3,Galactica, GPT4}. This can be reflected by their promising performances in biochemical QA and medical QA benchmarks \citep{GPT-4}.Therefore, it becomes urgent to leverage these LMs to assist chemistry and biology research.
% comment1: why we want to do this?
% comment2: show examples where LM can fail
% comment3: LM can fail in expert domains
Language Models (LMs) have demonstrated significant achievements across various domains~\citep{BERT, LLMSurvey}. Notably, the wealth of biochemical literature in LMs' pretraining data has enabled LMs to obtain a high-level understanding of biochemical concepts and molecule properties. This can be reflected by their promising performances in biochemical and medical question-answering benchmarks~\citep{Galactica,GPT4}. Therefore, it becomes increasingly urgent to incorporate these LMs to augment research in chemistry and biology.


% % context. The definition of molecule-language pretraining
% Para2: In this work, we study the task of molecule-language pretraining. molecule-language pretraining aims to bridge the modality gap between molecules and languages, in order to leverage the rich scientific knowledge and reasoning ability in LLMs for molecule understanding. It involves pretraining a multi-modal LM to understand both molecules and languages. This mulit-modal LM is later used for biochemistry tasks, including molecule retrieval, molecule captioning, and molecule property prediction~\citep{}. 
% In this work, we study Molecular Language Models (MolLMs). MolLM is a multi-modal LM that can achieve understand molecules and languages. It aims to bridge the modality gap between molecules and languages, in order to leverage the rich scientific knowledge and \yuan{reasoning ability} in LMs to assist chemistry research~\citep{KVPLM, MoleculeSTM}. It involves pretraining a multi-modal LM to understand both This mulit-modal LM is later used for multi-modal downstreams tasks, such as molecule-text retrieval~\citep{MoMu}, molecule captioning~\citep{MolT5}, and \yuan{language instructed molecule property prediction~\citep{Galactica}.}

% % review. Para3
% •	写法 1: The previous molecule-language pretrained methods can be categorized into two types. The first type represents molecules by their 1-d SMILES representations and process them as natural language. 
% •	写法 2: Most existing LMs represent molecules by their 1-d SMILES representations and process them as natural language~\citep{}. 
% In this way, the LM learns to associate the molecules' SMILES strings to their natural language context. However, representing molecules as strings is suboptimal for structure understanding and can cause xxx problem~\citep{}. To resolve the problem, recent works~\citep{MoMu and MoleculeSTM} represents molecules as graphs and use contrastive learning to bring together a graph encoder and a text encoder. These methods align the molecule representations to the output space of an LM, lead to promising retrieval performance.
% Figure: a) SMILES representation of molecules; b) align molecule representations to the output space of LLMs; c) ours: align molecule representations to the input space of LLMs.

% Most existing LMs represent molecules by their 1-dimensional SMILES strings~\citep{SMILES} and process them as natural language~\citep{Galactica, LLama}. 
% In this way, LMs \yuan{learn to associate the molecules' SMILES strings to their natural language context. However, representing molecules as strings is suboptimal for structure understanding and can cause xxx problem}. To resolve the problem, recent works~\citep{MoMu, MoleculeSTM} represents molecules as graphs and use contrastive learning to bring together a graph encoder and a text encoder. These methods align the molecule representations to the output space of an LM, lead to promising retrieval performance.

For this purpose, we aim to utilize LMs for molecule understanding. As shown in Figure~\ref{fig:framework_compare}a, most existing LMs~\citep{LLama, OPT, KVPLM} represent molecules by their 1D Simplified Molecular Input Line Entry System (SMILES) strings~\citep{SMILES} and process them in a manner similar to texts. While convenient, treating molecules as strings overlooks the molecules' 2D graph representations, which are crucial to human professionals in comprehending the molecule structures~\citep{wells2012structural}. To combat that, recent works~\citep{MoMu, MoleculeSTM} represent molecules as graphs and use a Graph Neural Network \citep[GNN;][]{xu2019powerful} as the molecule encoder. 
The GNN encoder is trained to align with an LM through cross-modal contrastive learning~\citep{CLIP,DeCLIP}, as illustrated in Figure~\ref{fig:framework_compare}b.
% Figure: a) SMILES representation of molecules; b) align molecule representations to the output space of LLMs; c) ours: align molecule representations to the input space of LLMs.
However, the application scope of cross-modal contrastive learning is limited, because it only provides a similarity score between a molecule and a text. 
This similarity score is suitable for retrieval tasks, but is insufficient for open-ended molecule-to-text generation tasks, such as molecule captioning~\citep{MolT5} and molecule's IUPAC name prediction~\citep{Galactica}. 
% This is because molecule-to-text generation requires the LM to understand the inputs of molecule representations
\yuan{This is because the LM is not trained for text generation when conditioned on the molecule input, and such training requires the \textbf{cross-modal alignment} between 2D graphs and 1D text.}
~\citet{MoMu} have explored adapting GNNs for text generation, however with limited performances.



\begin{figure*}[t]
 \centering
 \includegraphics[width=0.9\textwidth]{figures/framework_compare}
 \caption{Comparison of molecular language modeling methods.}
 \label{fig:framework_compare}
 \vspace{-10pt}
\end{figure*}


\begin{figure}[t]
 \centering\small
 \includegraphics[width=0.45\textwidth]{figures/pipeline}
 \caption{MolCA's three-stage training pipeline.}
 \vspace{-10pt}
\label{fig:pipeline}
\end{figure}









% This is because the LM is never trained for generation while conditioned on the \yuan{molecule representation (1D or 2D)}. MoMu~\citep{MoMu} has explored adapting a GNN encoder for molecule captioning, however with limited performances. 

% what is our work. How is it better than cross-modal contrastive learning
% To bridge the research gap, we introduce \textbf{MolCA}: \underline{Mol}ecular Graph-Language Modeling with \underline{C}ross-Modal Projector and Uni-Modal \underline{A}dapter. MolCA can interpret the inputs of both 2D molecular graphs and 1D texts, and can conduct open-ended molecule-to-text generation. As shown in Figure~\ref{fig:framework_compare}c, MolCA consists of three major components: 1) a graph encoder based on GNNs for understanding 2D molecular graphs, 2) an LM, integrated with a uni-modal adapter, for text generation and efficient downstream adaptation, and 3) \yuan{a cross-modal projector to bridge the modality gap between the graph encoder's representation space and the LM's input space.}
% \yuan{We believe the effective interplay between these components, as achieved by MolCA's three-stage training pipeline (Figure~\ref{fig:pipeline}), contributes to the success of molecule-to-text generation}. In this study, we assume the existence of effective graph encoder and LM that are pretrained in their respective domains. Under such context, the cross-modal projector and uni-modal adapter play vital roles in the three-stage training pipeline, thus allowing for the molecule-to-text generation. 

To bridge this gap, we devise \textbf{MolCA}: \underline{Mol}ecular Graph-Language Modeling with \underline{C}ross-Modal Projector and Uni-Modal \underline{A}dapter. It can understand the inputs of both 2D molecular graphs and 1D texts, so as to conduct open-ended molecule-to-text generation. As Figure~\ref{fig:framework_compare}c illustrates, MolCA consists of three major components: 1) a graph encoder based on GNNs for understanding 2D molecular graphs, 2) an LM, integrated with a uni-modal adapter, for text generation and efficient downstream adaptation, and 3) a cross-modal projector to bridge the modality gap between the graph encoder's representation space and the LM's input space. We believe the effective interplay between these components contributes to the success of molecule-to-text generation. In this study, we assume the existence of effective graph encoder and LM that are pretrained in their respective domains. Under such context, the cross-modal projector and the uni-modal adapter play vital roles in molecule-to-text generation. 
We now briefly introduce these two modules, and MolCA's training pipeline (cf. Figure~\ref{fig:pipeline}) for integrating its components. 



\textbf{Cross-Modal Projector.} The cross-modal projector is responsible for \textbf{cross-modal alignment}~\citep{BLIP2, LinearMapping, Flamingo}: to translate the graph encoder's outputs into soft prompts~\citep{PrefixTuning} in the text space so that the LM can understand. These soft prompts carry the structural information of the 2D molecular graphs. When conditioned on these prompts, the LM is able to generate better textual description about molecule structures. Inspired by the vision-language pretraining works~\citep{BLIP2}, we employ Querying Transformer (Q-Former) as the cross-modal projector. 
Q-Former performs cross-attention~\citep{Transformer} to extract molecule features from the graph encoder.


MolCA's two pretrain stages (Figure~\ref{fig:pipeline}) aim to optimize the cross-modal projector and the graph encoder for cross-modal alignment. In pretrain stage 1, the projector and the encoder are jointly trained to extract the molecule features that are relevant to the text.
% by cross-modal tasks of molecule-text contrasting, molecule-text matching, and molecule captioning~\citep{BLIP}. 
This stage endows the resulting model with powerful molecule-text retrieval ability. 
In pretrain stage 2, the cross-modal projector and the graph encoder are connected to a frozen LM and trained for molecule captioning. This stage forces the cross-modal projector to generate soft prompts that the LM can understand.


\textbf{Uni-Modal Adapter.} In the fine-tune stage, we adapt MolCA for downstream generation tasks. Considering that the LM accounts for a large portion of computation in MolCA, we employ a uni-modal adapter, LoRA~\citep{LoRA}, to improve the efficiency of the LM's fine-tuning. Specifically, LoRA adds new low-rank weight matrices in parallel to selected pretrained weights in the LM. We can then adapt the LM by fine-tuning only these new low-rank weights, which account for less than 1\% of the parameters in a 1.3B LM.

% \textbf{Uni-Modal Adapter.} The LM accounts for a large portion of computation in MolCA. Therefore, in the fine-tune stage, we employ a uni-modal adapter~\citep{Adapter} to improve the efficiency of the LM's downstream adaptation. We employ the LoRA~\citep{LoRA} adapter due to its simple implementation and promising performance~\citep{DBLP:conf/nips/LiuTMMHBR22}. 
% LoRA enables MolCA to be adapted for downstream tasks by fine-tuning only the adapter modules, which adds \yuan{1\%} parameters to a 1.3B LM.


% what can this work do? what is the performance?
We evaluate MolCA's cross-modal understanding ability in extensive downstream tasks, including molecule captioning~\cite{MolT5}, molecule retrieval~\cite{MoMu}, and molecule's IUPAC name prediction~\cite{Galactica}. 
We show that MolCA outperforms the existing state-of-the-art methods, including MoMu~\cite{MoMu}, MolT5~\cite{MolT5} and MoleculeSTM~\cite{MoleculeSTM}. \yuan{Moreover, our quantitative studies demonstrate that MolCA outperforms its base LM  in tests of probing molecule structures.}
% case studies showing MolCA that is capable of xxx. 

% Choose from:
% \begin{itemize}[leftmargin=*]
% \item Case studies on Molecule QA, such as "does the molecule have a ring?"; "what is the molecule's SMILES representations?", "what is the molecule's IUPAC name?"
% \item Experiments on few-shot learning and in-context learning.
% \item Case study on molecule generation by MoFlow.
% \end{itemize}

\begin{figure*}[t]
 \centering
 \includegraphics[width=0.9\textwidth]{figures/stage1}
 \caption{MolCA's pretrain stage 1. The graph encoder and the cross-modal projector (\ie Q-Former) are jointly optimized using three cross-modal tasks.  Modules of the same color share weights.}
 \label{fig:stage1}
 \vspace{-10pt}
\end{figure*}


